Internal Calculi for Separation Logics

We present a general approach to axiomatise separation logics with heaplet semantics with no external features such as nominals/labels. To start with, we design the first (internal) Hilbert-style axiomatisation for the quantifier-free separation logic. We instantiate the method by introducing a new separation logic with essential features: it is equipped with the separating conjunction, the predicate ls, and a natural guarded form of first-order quantification. We apply our approach for its axiomatisation. As a by-product of our method, we also establish the exact expressive power of this new logic and we show PSpace-completeness of its satisfiability problem.

==> section-core-formulae-capture-intervalSL.tex <==
In this section, we show that Boolean combinations of core formulae capture the expressive power of  \intervalSL. Therefore
aiming at axiomatising \intervalSL can be done, by axiomatising the Boolean combinations of core formulae as well as the process
of transforming any formula from \intervalSL into a logically equivalent Boolean combination of core formulae.
First, note that the atomic formulae of \intervalSL can be easily expressed as Boolean combinations of core formulae, as stated below.
\begin{itemize}
\item $\avariable = \avariablebis$ is already a core formula.
\item  $\avariable \Ipto \avariablebis$ is logically equivalent to
       $\seesgeq{\avariable}{\avariablebis}{\emptyset}{1} \land \lnot \seesgeq{\avariable}{\avariablebis}{\emptyset}{2}$.
\item $\emp$ is logically equivalent to $\lnot \remgeq{\emptyset}{1}$.
\end{itemize}

Lemma~\ref{lemma:star} below is a key result to guarantee that the set of core formulae introduced earlier is expressive enough
when the separating conjunction is involved. Its proof is similar to the proof of~\cite[Lemma 7]{DemriLM18}. Lemma~\ref{lemma:exists}
shall be in charge of the new operator with guarded existential quantification.

\begin{lemma}\label{lemma:star}
Suppose $\pair{\astore}{\aheap} \approx^\asetvar_{\bound} \pair{\astore'}{\aheap'}$. Then for all
$\bound_1,\bound_2 \in \Nat^+$ such that $\bound_1+\bound_2 = \bound$ and for all heaps $\aheap_1$, $\aheap_2$ such that $\aheap = \aheap_1 + \aheap_2$,
there are heaps
$\aheap'_1$, $\aheap'_2$ such that $\aheap' = \aheap'_1 + \aheap'_2$,
$\pair{\astore}{\aheap_1} \approx^\asetvar_{\bound_1} \pair{\astore'}{\aheap'_1}$ and
$\pair{\astore}{\aheap_2} \approx^\asetvar_{\bound_2} \pair{\astore'}{\aheap'_2}$.
\end{lemma}


\begin{proof}
\intextnote{SD}{check the proof of~\cite[Lemma 7]{DemriLM18} and either pinpoint the differences or
provide the adapted full developments.}
\end{proof}

Here comes the lemma for guarded existential quantification.

\begin{lemma}\label{lemma:exists}
Suppose $\pair{\astore}{\aheap} \approx^\asetvar_{2\bound} \pair{\astore'}{\aheap'}$. Given $\avariable,\avariablebis \in \asetvar$,
for any location $\alocation \in \minpath{\astore(\avariable)}{\astore(\avariablebis)}{\aheap} \cup \set{\astore(\avariablebis)}$,
there is a location $\alocation' \in \minpath{\astore'(\avariable)}{\astore'(\avariablebis)}{\aheap'} \cup \set{\astore'(\avariablebis)}$ such that for every $\avariableter \in \PVAR$,
$\pair{\astore[\avariableter \gets \alocation]}{\aheap} \approx^{\asetvar\cup\{\avariableter\}}_{\bound} \pair{\astore'[\avariableter \gets \alocation']}{\aheap'}$.
\end{lemma}

It is worth noting that there is substantial loss of precision when identifying a corresponding location in the other memory state.

\begin{proof} The proof is done by a case analysis depending on how $\alocation$ is related to the interpretation
of the terms from $ \atermset{\asetvar}$.
\begin{enumerate}
\item If there exists $\aterm \in \atermset{\asetvar}$ such that  $\semantics{\aterm}_{\astore,\aheap} = \alocation$, then
      $\alocation'$ takes the value $\semantics{\aterm}_{\astore',\aheap'}$.
\item Otherwise, there are two terms $\aterm_1,\aterm_2 \in \atermset{\asetvar}$ such that $\pair{\astore}{\aheap} \models \seesgeq{\aterm_1}{\aterm_2}{\asetvar\cup\ameetset{\asetvar}}{1}$
and $\alocation$ is such that there are $\alength_1,\alength_2 \geq 1$ $\aheap^{\alength_1}(\semantics{\aterm_1}_{\astore,\aheap}) = \alocation$ and $\aheap^{\alength_2}(\alocation) = \semantics{\aterm_2}_{\astore,\aheap}$ and
for every $\alength \in \interval{1}{\alength_1{+}\alength_2{-}1}$ $\aheap^{\alength}(\semantics{\aterm_1}_{\astore,\aheap}) \neq \semantics{\aterm_2}_{\astore,\aheap}$. Then,
\begin{itemize}
\item if $\alength_1 < \bound$, then select $\aheap^{\alength_1}(\semantics{\aterm_1}_{\astore',\aheap'})$ as $\alocation'$;
\item if $\alength_2 < \bound$, then select $\alocation'$ is the (only) location such that there is $\alength' \geq 1$ ${\aheap'}^{\alength'}(\semantics{\aterm_1}_{\astore',\aheap'}) = \alocation'$ and ${\aheap'}^{\alength_2}(\alocation') = \semantics{\aterm_2}_{\astore',\aheap'}$ and for every
$\alength \in \interval{1}{\alength'{+}\alength_2{-}1}$ ${\aheap'}^{\alength}(\semantics{\aterm_1}_{\astore',\aheap'}) \neq \semantics{\aterm_2}_{\astore',\aheap'}$.
\item otherwise $\alength_1 \geq \bound$ and $\alength_2 \geq \bound$. Then, $\alocation'$ takes the value $\aheap^{\bound}(\semantics{\aterm_1}_{\astore',\aheap'})$.
%% \qedhere
\end{itemize}
\end{enumerate}
Hence, for every $\avariableter \in \PVAR$,
$\pair{\astore[\avariableter \gets \alocation]}{\aheap} \approx^{\asetvar\cup\{\avariableter\}}_{\bound} \pair{\astore'[\avariableter \gets \alocation']}{\aheap'}$.
\end{proof}

The \defstyle{memory size} of a formula $\aformula$, written $\msize{\aformula}$, is defined inductively as follows.
\begin{multicols}{2}
\begin{itemize}
\item $\msize{\avariable = \avariablebis} \egdef \msize{\emp} = 1$
\item $\msize{\avariable \Ipto \avariablebis} \egdef 2$
\item $\msize{\aformulabis_1 \land \aformulabis_2} \egdef \max(\msize{\aformulabis_1},\msize{\aformulabis_2})$
\item $\msize{\lnot \aformulabis} \egdef \msize{\aformulabis}$
\item $\msize{\aformulabis_1 \separate \aformulabis_2} \egdef \msize{\aformulabis_1} + \msize{\aformulabis_2}$
\item $\msize{\inpath{\avariable}{\avariablebis}{\avariableter}\aformula} \egdef 2\times\msize{\aformula}$
\end{itemize}
\end{multicols}
Given a formula $\aformula$ with tree height $\alength$, $\msize{\aformula} \leq 2^{\alength+1}$.



\begin{theorem}
Let $\aformula$ be in \intervalSL.
Let $\asetvar \supseteq \freevars{\aformula}$ (set of program variables occurring in $\aformula$)
and $\bound \geq \msize{\aformula}$.
For all memory states $\pair{\astore}{\aheap}$ and $\pair{\astore'}{\aheap'}$ such that $\pair{\astore}{\aheap} \approx^\asetvar_\bound \pair{\astore'}{\aheap'}$,
we have $\pair{\astore}{\aheap} \models \aformula$ iff $\pair{\astore'}{\aheap'} \models \aformula$.
\end{theorem}

\begin{proof}
By structural induction we show that
 $\pair{\astore}{\aheap} \models \aformula$ iff $\pair{\astore'}{\aheap'} \models \aformula$.
It is sufficient to establish one direction of the equivalence thanks to its symmetry.

The basic cases for the atomic formulae are immediate.
We omit the obvious cases with the Boolean connectives.

Let us consider the case $\aformula = \aformulabis_1 \separate \aformulabis_2$.
Suppose that $\pair{\astore}{\aheap} \models \aformulabis_1 \separate \aformulabis_2$.
Then, there are heaps $\aheap_1$ and $\aheap_2$ such that
$\aheap = \aheap_1 + \aheap_2$,
$\pair{\astore}{\aheap_1} \models \aformulabis_1$
and $\pair{\astore}{\aheap_2} \models \aformulabis_2$.
As $\bound \geq \msize{\aformulabis_1 \separate \aformulabis_2} = \msize{\aformulabis_1} + \msize{\aformulabis_2}$,
there exist $\bound_1$ and $\bound_2$ such that $\bound = \bound_1 + \bound_2$,
$\bound_1 \geq \msize{\aformulabis_1}$ and $\bound_2 \geq \msize{\aformulabis_2}$.
By Lemma~\ref{lemma:star},
there exist heaps $\aheap'_1$ and $\aheap'_2$ such that
      $\aheap'=\aheap'_1 + \aheap'_2$,
      $\pair{\astore}{\aheap_1} \approx^\asetvar_{\bound_1}  \pair{\astore'}{\aheap'_1}$ and
      $\pair{\astore}{\aheap_2} \approx^\asetvar_{\bound_2}  \pair{\astore'}{\aheap'_2}$.
      By the induction hypothesis, we get  $\pair{\astore'}{\aheap_1'} \models \aformulabis_1$
and $\pair{\astore'}{\aheap_2'} \models \aformulabis_2$. Consequently, we obtain
$\pair{\astore'}{\aheap'} \models \aformulabis_1 \separate \aformulabis_2$.

Lastly, we consider the case $\aformula = \inpath{\avariable}{\avariablebis}{\avariableter} \aformulabis$.
Suppose that $\pair{\astore}{\aheap} \models \inpath{\avariable}{\avariablebis}{\avariableter} \aformulabis$.
Then, there is $\alocation \in \minpath{\astore(\avariable)}{\astore(\avariablebis)}{\aheap} \cup \set{\astore(\avariablebis)}$ such that
$\pair{\astore[\avariableter \gets \alocation]}{\aheap} \models \aformulabis$.
As $\bound \geq \msize{\inpath{\avariable}{\avariablebis}{\avariableter} \aformulabis} = 2\times\msize{\aformulabis}$, by Lemma~\ref{lemma:reducebound},
 we obtain $\pair{\astore}{\aheap} \approx^\asetvar_{2\times\msize{\aformulabis}} \pair{\astore'}{\aheap'}$.
By Lemma~\ref{lemma:exists}, there exists $\alocation' \in \minpath{\astore'(\avariable)}{\astore'(\avariablebis)}{\aheap'} \cup \set{\astore'(\avariablebis)}$ such that
for every $\avariablefour \in \PVAR$ $\pair{\astore[\avariablefour \gets \alocation]}{\aheap} \approx^{\asetvar\cup\{\avariablefour\}}_{\msize{\aformulabis}} \pair{\astore'[\avariablefour \gets \alocation']}{\aheap'}$.
As $\asetvar \supseteq \freevars{\aformula}$, by definition we obtain $\asetvar \cup \{\avariableter\} \supseteq \freevars{\aformulabis}$. Then, by
the induction hypothesis $\pair{\astore'[\avariableter \gets \alocation']}{\aheap'} \models \aformulabis$.
As the location $\alocation'$ is in $\minpath{\astore'(\avariable)}{\astore'(\avariablebis)}{\aheap'}  \cup \set{\astore'(\avariablebis)}$,
 and is such that $\pair{\astore'[\avariableter \gets \alocation']}{\aheap'} \models \aformulabis$,
by definition of $\models$, we conclude that $\pair{\astore'}{\aheap'} \models \inpath{\avariable}{\avariablebis}{\avariableter} \aformulabis$.
\end{proof}


\begin{corollary}
\label{corollary:boolean-combinations}
Let $\aformula$ be in \intervalSL. There is a Boolean combination $\aformulabis$ of core formulae
from $\coreformulae{\freevars{\aformula}}{\msize{\aformula}}$ that is logically equivalent to $\aformula$.
\end{corollary}

A substantial part of the axiomatisation (but not the only involved part) is dedicated to
compute such  logically equivalent Boolean combinations of core formulae, when the core formulae
are understood as abbreviations in \intervalSL.

